Contact-Aware Non-prehensile Robotic Manipulation for Object Retrieval in Cluttered Environments

Non-prehensile manipulation methods usually use a simple end effector, e.g., a single rod, to manipulate the object. Compared to the grasping method, such an end effector is compact and flexible, and hence it can perform tasks in a constrained workspace; As a trade-off, it has relatively few degrees of freedom (DoFs), resulting in an under-actuation problem with complex constraints for planning and control. This paper proposes a new non-prehensile manipulation method for the task of object retrieval in cluttered environments, using a rod-like pusher. Specifically, a candidate trajectory in a cluttered environment is first generated with an improved Rapidly-Exploring Random Tree (RRT) planner; Then, a Model Predictive Control (MPC) scheme is applied to stabilize the slider's poses through necessary contact with obstacles. Different from existing methods, the proposed approach is with the contact-aware feature, which enables the synthesized effect of active removal of obstacles, avoidance behavior, and switching contact face for improved dexterity. Hence both the feasibility and efficiency of the task are greatly promoted. The performance of the proposed method is validated in a planar object retrieval task, where the target object, surrounded by many fixed or movable obstacles, is manipulated and isolated. Both simulation and experimental results are presented.

==> chapters/4_method.tex <==


In this section, we provide the formulation of the dynamic reinforcement learning (dynamic RL) framework, 
%
including some definitions of dynamic RL (Sec.~\ref{sec: def of dyrl}),
%
derivation of the dynamic Markov decision process (dynamic MDP) (Sec.~\ref{sec: derivation of dymdp}), 
%
and further prove the convergence of value iteration of dynamic MDP theoretically (Sec.~\ref{sec: convergency}). 
%
Finally we give a practical implementation of dynamic RL based on a commonly-used RL algorithm, \textit{i.e.}, TD3 \cite{fujimoto2018TD3} (Sec.~\ref{sec: practical implementation}).

\subsection{Efficient Sampling-based Planning in Clutter} \label{sec: def of dyrl}


\subsection{Derivation of Robust Pushing Controller} \label{sec: derivation of dymdp}
\vspace{-3pt}
\textcolor{red}{The MPC-based pushing controller is augmented with Disturbance Observer (DOB) to stabilize the slider's trajectory under potential contacts and parameter uncertainties. We model the system's dynamics as
\begin{equation}
    \dot{x}(t)=f(x(t),u(t))+d(t),
\end{equation}
where $x(t), u(t)$ are state and input vectors, $f(\cdot)$ is the nonlinear function, and $d(t)$ represents the disturbance. Discretize the dynamics at timestep $k$ and we get
\begin{equation}
    \hat{x}_{k+1}=x_k+dt\cdot\left[f(x_k,u_k)+\hat{d}\right].
\end{equation}
Here $\hat{d}$ is the estimated disturbance with update law
\begin{equation}
    \dot{\hat{d}}_k=\beta\cdot(x_{k+1}-\hat{x}_{k+1}),
\end{equation}
where $x_{k+1}, \hat{x}_{k+1}$ are observed and predicted states, and $\beta>0$ denotes the update rate.}

The MPC-based pushing controller is augmented with Disturbance Observer (DOB) to stabilize the slider's trajectory under potential contacts and parameter uncertainties. The pusher-slider motion is formalized as the following nonlinear affine system
\begin{equation}
\begin{aligned}
\dot {\bm x} &= \bm g_1(\bm x)\bm u + \bm g_2(\bm x)\bm d 
  \\ 
 & = \left[\begin{array}{ccc}
    \bm R\bm L \bm J_C^\top & 0 & 0 \\
     0& 1&-1
\end{array}\right] \bm u + \left[\begin{array}{c}
     \bm R \\
     0
\end{array}\right] \bm d,
\end{aligned}
\end{equation}
where the lumped disturbance vector $\bm d \in \mathbb{R}^3$ is assume to lump the effect of unknown contact wrenches and uncertain slider coefficients. The disturbance vector $\bm d$ satisfies the matching condition, which means there exists a smooth function $g_d(\bm x)$ such that $g_1(\bm x)g_d(\bm x) = g_2(\bm x)$. The estimated disturbance $\hat{\bm d}$ is updated by 
\begin{equation}
      \dot {\hat {\bm d}} = \bm K_d \hat{\bm d}  + \bm L_d(\bm x)\dot {\bm x} - \bm L_d(\bm x) \bm g_1(\bm x)\bm u,
\end{equation}
where the disturbance gain matrix $\bm K_d $ is positive diagonal matrix, and state gain matrix $\bm L_d(\bm x)$ is proposed as 
\begin{equation}
    \bm L_d(\bm x) = \bm K_d g_2^{\dagger}(\bm x).
\end{equation}
In order to compensating the disturbance, the control input $\bm u$ is designed for the estimated system
\begin{equation}
    \dot {\bm x} = \bm g_1(\bm x)\bm u + \bm g_2(\bm x) \hat{\bm d},
\end{equation}
using the model predictive controller under the MPCC\cite{}
\begin{comment}
\textcolor{black}{In order to compensating the disturbance, the following DOB-based control input at time step k is considered
\begin{equation}
    \bm u_k = \bm u_{nk} -g_d(\bm x_k) \hat{\bm d}_k,
\end{equation}
where the nominal control input $\bm u_{nk}$ is designed for the nominal system without disturbances, using a model predictive controller under the MPCC\cite{}, and the estimated disturbance \hat{\bm d} is updated by 
\begin{equation}
      \hat {\bm d}_{k+1} = \left(I- {\Delta} t\bm K_d\right) \hat{\bm d}_k  + \bm L_d(\bm x_k)\left(x_k -x_{nk}\right),
\end{equation}
where the disturbance gain matrix $\bm K_d $ is positive diagonal matrix, and state gain matrix $\bm L_d(\bm x)$ is proposed as 
\begin{equation}
    \bm L_d(\bm x) = \bm K_d g_2^{\dagger}(\bm x).
\end{equation}}
\end{comment}
